Supervised Learning with Similarity Functions

We address the problem of general supervised learning when data can only be accessed through an (indefinite) similarity function between data points. Existing work on learning with indefinite kernels has concentrated solely on binary/multi-class classification problems. We propose a model that is generic enough to handle any supervised learning task and also subsumes the model previously proposed for classification. We give a "goodness" criterion for similarity functions w.r.t. a given supervised learning task and then adapt a well-known landmarking technique to provide efficient algorithms for supervised learning using "good" similarity functions. We demonstrate the effectiveness of our model on three important super-vised learning problems: a) real-valued regression, b) ordinal regression and c) ranking where we show that our method guarantees bounded generalization error. Furthermore, for the case of real-valued regression, we give a natural goodness definition that, when used in conjunction with a recent result in sparse vector recovery, guarantees a sparse predictor with bounded generalization error. Finally, we report results of our learning algorithms on regression and ordinal regression tasks using non-PSD similarity functions and demonstrate the effectiveness of our algorithms, especially that of the sparse landmark selection algorithm that achieves significantly higher accuracies than the baseline methods while offering reduced computational costs.

==> NIPS Camera Ready/intro.tex <==
\section{Introduction}
The goal of this paper is to develop an extended framework for supervised learning with similarity functions. Kernel learning algorithms \cite{kernel-book} have become the mainstay of discriminative learning with an incredible amount of effort having been put in, both from the theoretician's as well as the practitioner's side. 
% with several theoretical results providing generalization guarantees as well as from the practitioners side with several \emph{off-the-shelf} toolkits available for various kernel learning problems. 
However, these algorithms typically require the similarity function to be a positive semi-definite (PSD) function, which can be a limiting factor for several applications. Reasons being: 1) the Mercer's condition is a formal statement that is hard to verify, 2) several natural notions of similarity that arise in practical scenarios are not PSD, and 3) it is not clear as to why an artificial constraint like PSD-ness should limit the usability of a kernel. 

Several recent papers have demonstrated that indefinite similarity functions can indeed be successfully used for learning \cite{feature-svm-indef,learn-indef,learn-kern-from-indef,svm-indef}. However, most of the existing work focuses on classification tasks and provides specialized techniques for the same, albeit with little or no theoretical guarantees. A notable exception is the line of work by \cite{learn-sim,learn-dissim,dissim-nips} that defines a goodness criterion for a similarity function and then provides an algorithm that can exploit this goodness criterion to obtain provably accurate classifiers. However, their definitions are yet again restricted to the problem of classification as they take a ``margin'' based view of the problem that requires positive points to be more similar to positive points than to negative points by at least a constant margin. 

In this work, we instead take a ``target-value'' point of view and require that target values of similar points be similar. Using this view, we propose a generic goodness definition that also admits the goodness definition of \cite{learn-sim} for classification as a special case. Furthermore, our definition can be seen as imposing the existence of a smooth function over a generic space defined by similarity functions, rather than over a Hilbert space as required by typical goodness definitions of PSD kernels. 

We then adapt the landmarking technique of \cite{learn-sim} to provide an efficient algorithm that reduces learning tasks to corresponding learning problems over a linear space. The main technical challenge at this stage is to show that such reductions are able to provide good generalization error bounds for the learning tasks at hand. To this end, we consider three specific problems: a) regression, b) ordinal regression, and c) ranking. For each problem, we define appropriate surrogate loss functions, and show that our algorithm is able to, for each specific learning task, guarantee bounded generalization error with polynomial sample complexity. Moreover, by adapting a general framework given by \cite{kernel-sim-compare}, we show that these guarantees do not require the goodness definition to be overly restrictive by showing that our definitions admit all good PSD kernels as well.

%but are required to adapt it to each individual supervised learning task that we consider. 

For the problem of real-valued regression, we additionally provide a goodness definition that captures the intuition that usually, only a small number of landmarks are influential w.r.t. the learning task. However, to recover these landmarks, the uniform sampling technique would require sampling a large number of landmarks thus increasing the training/test time of the predictor. We address this issue by applying a sparse vector recovery algorithm given by \cite{acc-sparse} and show that the resulting sparse predictor still has bounded generalization error.   %allows us to prune away irrelevant features in the landmarking stage. To avoid getting stuck with a hard combinatorial problem, 
%for a few influential landmarks, however selecting these small number of landmarks become a combinatorial problem. To alleviate this issue, 
%we apply a sparse vector recovery algorithm 
%Fully Corrective Forward Selection method 
%by \cite{acc-sparse} and show generalization error bounds for the same.

We also address an important issue faced by algorithms that use landmarking as a feature constructions step viz \cite{learn-sim,learn-dissim,dissim-nips}, namely that they typically assume separate landmark and training sets for ease of analysis. In practice however, one usually tries to overcome paucity of training data by reusing training data as landmark points as well. We use an argument outlined in \cite{double-dipping} to theoretically justify such
``double dipping'' in our case. The details of the argument are given in \ref{app:double-dipping}.

We perform several experiments on benchmark datasets that demonstrate significant performance gains for our methods over the baseline of kernel regression. Our sparse landmark selection technique provides significantly better predictors that are also more efficient at test time. %offers especially attractive results at reduced computational costs. 

%{\color{red} Finally, we conduct experiments on benchmark datasets using non-PSD kernels for regression and ordinal regression tasks. We compare our methods against a standard baseline of kernel regression {\large {\bf that is commonly used heuristic when kernels are non-PSD}}. For both the tasks, we show that our methods are significantly better than the baseline and provide predictions using a small number of similarity function computation at the test time.
%Moreover, we show that our sparse landmark selection technique further reduces the number of landmarks required while maintaining similar or sometimes even better accuracy than the random landmark selection method.}

{\bf Related Work}: Existing approaches to extend kernel learning algorithms to indefinite kernels can be classified into three broad categories: a) those that use indefinite kernels directly with existing kernel learning algorithms, resulting in non-convex formulations \cite{feature-svm-indef,learn-indef}. %This results in non-convex formulations 
%with a proliferation of local minima with no useful generalization guarantees. Moreover 
%that require customized stabilization routines to be written.
% for these algorithms. 
 b) those that convert a given indefinite kernel into a PSD one by either projecting onto the PSD-cone \cite{learn-kern-from-indef,svm-indef} or performing other spectral operations \cite{classfn-sim}. The second approach is usually expensive due to the spectral operations involved apart from making the method inherently transductive. 
% The spectral projections involved are usually task oblivious and expensive to carry out. But most importantly, 
 Moreover, any domain knowledge stored in the original kernel is lost due to these task oblivious operations and consequently, no generalization guarantees can be given.
% these approaches the domain knowledge stored in the similarity function can be lost due to these operations and consequently one is unable to provide any useful generalization guarantees. 
 c) those that use notions of ``task-kernel alignment'' or equivalently, notions of ``goodness'' of a kernel, to give learning algorithms 
% to convert the similarity-based learning problem into a PSD kernel learning problem 
 \cite{learn-sim,learn-dissim,dissim-nips}. This approach enjoys several advantages over the other approaches listed above. These models are able to use the indefinite kernel directly with existing PSD kernel learning techniques; all the while retaining the ability to give generalization bounds that 
% ere are several advantages to this approach: first of all the similarity function is unmodified hence domain knowledge is preserved, secondly, there are models of learning which offer generalization guarantees that 
 quantitatively parallel those of PSD kernel learning models. In this paper, we adopt the third approach for general supervised learning problem. %This is the approach taken by the present paper as well.
% Moreover, the algorithms that these models offer allow us to use existing solvers for learning with indefinite kernels as well. In our work, we take an approach similar to the last approach and generalize the same to general supervised learning tasks. 
%However, the last line of work has, so far, only concentrated on classification problems. Our goal in this paper is to extend this line of work to other supervised learning problems. A key ingredient in our approach is the notion of ``goodness'' of a similarity function. Informally, a similarity function is called ``good'' for a classification task if it does not cluster oppositely labeled points together. In other words, positively labeled points should, on an average, be more similar to other positively labeled points than to negatively labeled points and vice-versa. At first glance this seems like a very natural condition and indeed, as results of \cite{kernel-sim-compare} show, for the case of PSD kernels, this is equivalent to having a large margin in the RKHS.
%The first hurdle one faces while extending this model beyond classification-like tasks is the absence of a notion of \emph{labels}. Our first task, therefore, is to provide a more general notion of goodness that is suitable for learning tasks such as regression, ordinal regression and ranking. We give this definition below.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dissim"
%%% End: 

